Intriguing Properties of Data Attribution on Diffusion Models

Data attribution seeks to trace model outputs back to training data. With the recent development of diffusion models, data attribution has become a desired module to properly assign valuations for high-quality or copyrighted training samples, ensuring that data contributors are fairly compensated or credited. Several theoretically motivated methods have been proposed to implement data attribution, in an effort to improve the trade-off between computational scalability and effectiveness. In this work, we conduct extensive experiments and ablation studies on attributing diffusion models, specifically focusing on DDPMs trained on CIFAR-10 and CelebA, as well as a Stable Diffusion model LoRA-finetuned on ArtBench. Intriguingly, we report counter-intuitive observations that theoretically unjustified design choices for attribution empirically outperform previous baselines by a large margin, in terms of both linear datamodeling score and counterfactual evaluation. Our work presents a significantly more efficient approach for attributing diffusion models, while the unexpected findings suggest that at least in non-convex settings, constructions guided by theoretical assumptions may lead to inferior attribution performance. The code is available at https://github.com/sail-sg/D-TRAK.

==> sections/07_Related.tex <==
\section{Related work}

\textbf{TDA} There is a sizeable body of work on data attribution methods. 
Here we discuss approaches most similar to ours, but we refer the reader to \citet{hammoudeh2022training} for an even more extensive survey.
A major line of works uses \emph{Hessian-based Influence Functions} for data attribution~\cite{koh2017understanding}.
In particular, the influence function effectively computes--up to an error that can be bounded--the one-step Newton approximation with respect to the full model parameters~\cite{koh2019accuracy}.
\citet{pruthi2020estimating} further propose TracInCP.
\citet{kong2021understanding} adapt Influence Functions and TracInCP to VAE~\citep{kingma2013auto}.
\citet{terashita2021influence} adapt Influence Functions to GAN~\citep{goodfellow2020generative}.

\textbf{Concurrent Work} \cite{georgiev2023journey} also adapt TRAK to diffusion models (one of the baselines). 
\cite{dai2023training} use machine unlearning method (not post-hoc).
\cite{wang2023evaluating} use extra datasets and tune models such as DINO, CLIP, and ViT to improve the image similarity quality (not evaluating faithfulness but plausibility, which is not what we want, need to construct extra data and only consider text-to-image models). 

==> sections/09_Intro_practice.tex <==
%%%% try to write an introduction
Training data attribution analyzes how changes to the training data can result in different model predictions and helps investigate questions such as, ``how would this prediction change if I were to \emph{remove} these training examples''.

With the recent development of generative tasks enabled by large-scale diffusion models, data attribution becomes a desired module to properly assign valuations for high-quality or copyrighted training samples, ensuring that data contributors are fairly compensated or credited. 

Data attribution has been extensively studied for discriminative tasks such as classification~\citep{koh2017understanding}. 
Several advanced methods have been proposed to implement data attribution, primarily motivated by theoretical analyses, in an effort to improve the trade-off between computational scalability and effectiveness~\citep{park2023trak}. 

In this study, we initially try to conduct data attribution on diffusion guided by the above methods which are theoretically justified under the convex settings.

Intriguingly, we fortuitously observe that theoretically \emph{unjustified} design choices for attribution empirically outperform previous baselines by a large margin in terms of both linear datamodeling score and counterfactual predictions. 

Surround this counter-intuitive observation, we conduct extensive experiments and ablation studies on attributing diffusion models, specifically focusing on DDPMs trained on CIFAR-10 and CelebA, as well as a Stable Diffusion model LoRA-finetuned on ArtBench. 

Our work presents a significantly more efficient approach for attributing diffusion models, while the unexpected findings suggest that at least in the non-convex settings, constructions guided by theoretical assumptions may lead to inferior attribution performance.
